Streamlining the review process: AI-generated annotations in research manuscripts

The increasing volume of research paper submissions poses a significant challenge to the traditional academic peer-review system, leading to an overwhelming workload for reviewers. This study explores the potential of integrating Large Language Models (LLMs) into the peer-review process to enhance efficiency without compromising effectiveness. We focus on manuscript annotations, particularly excerpt highlights, as a potential area for AI-human collaboration. While LLMs excel in certain tasks like aspect coverage and informativeness, they often lack high-level analysis and critical thinking, making them unsuitable for replacing human reviewers entirely. Our approach involves using LLMs to assist with specific aspects of the review process. This paper introduces AnnotateGPT, a platform that utilizes GPT-4 for manuscript review, aiming to improve reviewers' comprehension and focus. We evaluate AnnotateGPT using a Technology Acceptance Model (TAM) questionnaire with nine participants and generalize the findings. Our work highlights annotation as a viable middle ground for AI-human collaboration in academic review, offering insights into integrating LLMs into the review process and tuning traditional annotation tools for LLM incorporation.

==> relatedWork.tex <==

\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Reference} & \textbf{Aim} & \textbf{Intervention} & \textbf{Results} \\
\hline
ghosal2019deepsentipeer & proposes & - & - \\
\hline
checco2021ai & introduces & - & However, the researchers also acknowledge the importance of addressing potential biases and ethical concerns associated with these tools. \\
\hline
wang2020reviewrobot & introduces & Experimental results demonstrate that this review score predictor achieves an accuracy ranging from 71.4\% to 100\% in the domains of NLP and ML. & Experimental results demonstrate that this review score predictor achieves an accuracy ranging from 71.4\% to 100\% in the domains of NLP and ML. \\
\hline
yuan2022can & introduces & - & - \\
\hline
Penelope.ai & - & - & - \\
\hline
srivastava2023day & introduces & - & - \\
\hline
biswas2023focus & investigate & - & - \\
\hline
\end{tabular}

==> requirementTable.tex <==

\begin{table}[!ht]
\caption{Annotation-Driven Concept Mapping: Tool Requirements.}
\begin{tabular}{|c|p{3cm}|p{3cm}|p{2.5cm}|p{4.2cm}|}
    \hline
     & \textbf{Activity} & \textbf{Aim} & \textbf{Stakeholder} & \textbf{Tool Requirement} \\
    \hline
    R1 & \makecell{Concept \\ Mapping} & capture the concept map & the learner & draw nodes and arcs \\
    \hline
    R2 & \makecell{Learning \\ from text} & keep the reading flow & the learner & capture concepts/relations while reading \\
    \hline
    R3 & \makecell{Learning \\ from text} & strategic reading & the learner &  annotation based on constructs from the concept map \\
    \hline
    R4 & \makecell{Feedback \\ provision} & contextualized feedback & the instructor & support for categories   \\    
    \hline
    R5 & \makecell{Feedback \\ provision} & specific feedback & the instructor & support for annotations  \\
    \hline
    R6 & \makecell{Feedback \\ provision} & timely feedback & the instructor  & transparent migration of annotations  \\
    \hline
\end{tabular}
\label{tab:requirements}
\end{table}






==> swot.tex <==


\begin{table}[h]
\centering
\caption{SWOT Analysis}
\begin{tabular}{ | m{0.5\textwidth} | m{0.5\textwidth} | }
\hline
\textbf{Strengths} & \textbf{Weaknesses} \\
\hline
\begin{itemize}
    \item Manuscript reviewing process
    \item Summarizing, extracting key points
    \item Identifying potential issues
    \item Consistency in review process
    \item Growing workload management
\end{itemize} & 
\begin{itemize}
    \item Contextual understanding
    \item Semantic coherence
    \item Originality and creativity assessment
    \item Intent interpretation
    \item Replicability
    \item Sensitivity to prompts
\end{itemize} \\
\hline
\textbf{Opportunities} & \textbf{Threats} \\
\hline
\begin{itemize}
    \item Rigor and validity in peer-reviews
    \item Analysis of published articles
    \item Highlighting related works
    \item Suggesting improvements
    \item Identifying research gaps
    \item Speeding up peer-review
    \item Reducing biases
    \item Translation and language assistance
    \item Accessible feedback
\end{itemize} & 
\begin{itemize}
    \item Ethical concerns
    \item Data privacy
    \item Bias and misuse
    \item Sensitive information protection
    \item Overreliance on AI
    \item Technical limitations
    \item Noise in generated text
    \item Sensitivity to input variations
\end{itemize} \\
\hline
\end{tabular}
\label{tab:swot}
\end{table}



